Experimentation With Fuzzy Interest Forwarding in Named Data Networking

In the current Named Data Networking implementation, forwarding a data request requires finding an exact match between the prefix of the name carried in the request and a forwarding table entry. However, consumers may not always know the exact naming, or an exact prefix, of their desired data. The current approach to this problem-establishing naming conventions and performing name lookup-can be infeasible in highly ad hoc, heterogeneous, and dynamic environments: the same data can be named using different terms or even languages, naming conventions may be minimal if they exist at all, and name lookups can be costly. In this paper, we present a fuzzy Interest forwarding approach that exploits semantic similarities between the names carried in Interest packets and the names of potentially matching data in CS and entries in FIB. We describe the fuzzy Interest forwarding approach, outline the semantic understanding function that determines the name matching, and present our simulation study along with extended evaluation results.

==> 5-challenges.tex <==
\section{System Implementation Considerations/Challenges}
\label{sec:challenges}

While there are some clear benefits to implementing FIF into NDN, there are various challenges to address with regard to implementation and design approaches.   We identify approaches and tradeoffs in the implementation of fuzzy matching within the NDN forwarding process. 

\paragraph{Resource Constraints} Currently, the semantic similarity function (as described in Section \ref{sec:fuzzynamematching}) is large in terms of its storage and computation demands, consuming a lot of resources and take a long time to produce results. In a highly resource-constrained network environment, we may assume a centralized service (i.e., semantic oracle) that provides the semantic analysis required to perform each step of the fuzzy forwarding process. This pushes the computational and storage cost to the individual NDN nodes, but provides the FIF capability if adequate network bandwidth is available. In the bandwidth limited environment, we may consider other approaches to perform a fast, but possibly lower performing approach to locally perform fuzzy matching. Some potential approaches are to use a Locality-Sensitive Hash (LSH) to coarsely identify semantically similar data or Interests. Given these overall resource constraints in the dynamic network environment, we may choose to have not all forwarders have to have the fuzzy matching processes, where non-fuzzy nodes will perform forwarding according to the default NDN nodes.

\textit{Unsorted Snippets}
\begin{itemize}
\item Reality-check: Memory requirements (TCAM, Hash tables, Bloom filters, etc. etc.) Speed.
\item nodes within local vicinity can learn from each other what info they just obtained (e.g., a sensor measured an explosion, a camera noticed a new fast moving target, or a group split into two??).  This would make FF very useful in environment with highly dynamic changes, addresses the issues of b) and c) mentioned above. 
\item Threshold fuzzy matching:  Use locality-sensitive bloom filter; recursively at each level of name hierarchy?
\item Memory requirements (TCAM, Hash tables, Bloom filters, etc. etc.) Speed.
\end{itemize}

%\subsection{Worked Example}
%We present a toy example to demonstrate how we envision fuzzy information forwarding to perform given uncertainty in the namespace. While the named data in actual networks will be much larger, we use an example dataset taken from the UCI Machine Learning Repository Zoo Data Set \cite{Lichman2013uci}. We use the Synset in WordNet \cite{Fellbaum1998wordnet} corpus and use the WUP Similarity score as the semantic similarity function. We assume the situation where a user from another network of related domain has access to another named data network. FIF is used to provide semantically similar named data and information about the namespace design. Based on the available network resources, the threshold $\tau$ can be adapted. Given an increasing value of $\tau$, we see additional names or named data returned through the fuzzy matching or forwarding process. Figure \ref{fig:names_vs_tau} shows the increase of names returned to the source of the interest as a result of FIF. We see that a sharp transition at around $\tau = .3$. This is obviously dependent on the specific tag and corpus/namespace.
%
%\begin{figure}
%  \includegraphics[width=\linewidth]{names_vs_tau.pdf}
%  \caption{Names vs $\tau$ using WUP over the Wordnet Synset corpora matching wildebeast to the UCI Zoo dataset.}
%  \label{fig:names_vs_tau}
%\end{figure}
%
%\begin{figure}[!htb]
%     \centering
%     \subfigure[Comparison of query response time] {
%        \label{fig:lsh-time}
%        \includegraphics[width=.47\textwidth]{./figures/lsh_time_d400.pdf}}
%    \subfigure[Accuracy of LSH Forest method for nearest neighbor search] {
%        \label{fig:lsh-accuracy}
%        \includegraphics[width=.47\textwidth]{./figures/lsh_accuracy_d400.pdf}}
%    \caption{Performance of approximate nearest neighbor search using LSH Forest algorithm (400-dimensional vectors)}
%    \label{fig:lsh-performance}
%\end{figure}
%
%As a proof point for efficient methods for fuzzy name look-up, we conduct an experiment to measure the performance of an approximate nearest neighbor (ANN) search using LSH Forest~\cite{bawa2005lsh} method for 400-dimensional vector space. The results are shown in Figure~\ref{fig:lsh-performance}. In Figure~\ref{fig:lsh-time}, we compare the NN query response times of LSH Forest method with different parameters against a brute-force linear search as we vary in the $x$-axis the total number of data points to which the given query vector is to be compared against. Figure~\ref{fig:lsh-accuracy} shows the average accuracy of the ANN search result returned by LSH Forest method. Overall, these results indicate that LSH Forest method (or other ANN methods) can produce reasonably accurate NN search results with almost constant search response time (subject to the tuning of the parameters in the tradeoff space of complexity vs. accuracy), making them viable choices for fuzzy name search mechanisms in resource-constrained NDN routers.

==> Makefile <==
PRJ = fuzzyfwd

# Small cheat to allow synchronization between PDF and .tex for supported editors (run `make S=1`)
ifdef S
EXTRA = -synctex=1
endif

all : ${PRJ}.pdf

${PRJ}.pdf : *.tex *.bib
	pdflatex ${EXTRA} ${PRJ} && \
		(ls ${PRJ}.aux | xargs -n 1 bibtex) && \
		pdflatex ${EXTRA} ${PRJ} && pdflatex ${EXTRA} ${PRJ}

view : ${PRJ}.pdf
	open ${PRJ}.pdf &

clean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log *~* *.bak *.out *synctex.gz *.dvi *.rel ${PRJ}.pdf cut.sh

